A Survey on Federated Fine-tuning of Large Language Models

Large Language Models (LLMs) have demonstrated impressive success across various tasks. Integrating LLMs with Federated Learning (FL), a paradigm known as FedLLM, offers a promising avenue for collaborative model adaptation while preserving data privacy. This survey provides a systematic and comprehensive review of FedLLM. We begin by tracing the historical development of both LLMs and FL, summarizing relevant prior research to set the context. Subsequently, we delve into an in-depth analysis of the fundamental challenges inherent in deploying FedLLM. Addressing these challenges often requires efficient adaptation strategies; therefore, we conduct an extensive examination of existing Parameter-Efficient Fine-tuning (PEFT) methods and explore their applicability within the FL framework. To rigorously evaluate the performance of FedLLM, we undertake a thorough review of existing fine-tuning datasets and evaluation benchmarks. Furthermore, we discuss FedLLM's diverse real-world applications across multiple domains. Finally, we identify critical open challenges and outline promising research directions to foster future advancements in FedLLM. This survey aims to serve as a foundational resource for researchers and practitioners, offering valuable insights into the rapidly evolving landscape of federated fine-tuning for LLMs. It also establishes a roadmap for future innovations in privacy-preserving AI. We actively maintain a \href{https://github.com/Clin0212/Awesome-Federated-LLM-Learning}{GitHub repo} to track cutting-edge advancements in this field.

==> TMLR_Survey/Figs/Figure_memory_wall.tex <==
  %----------------------------------------------
  \begin{figure}
    \centering
    \begin{tikzpicture}
    \normalsize{
    \scriptsize{
      \begin{axis}[
      at={(0em,0em)},
    ymajorgrids=true,
        xmajorgrids=true,
        grid style=dashdotted,
        ybar,
        enlarge x limits=0.2,
        height=.7\linewidth,
        width=1.0\linewidth,
        bar width=1.8em,
        symbolic x coords = {{ASQA},{ELI5},{QAMPARI}},
        ymin=10,
        ymax=70,
        ytick = {20,30,40,50,60},
        ylabel={Citation F1(\%)},
        xtick = data,
        xticklabel style={/pgf/number format/fixed,/pgf/number format/fixed zerofill,/pgf/number format/precision=1},
        legend style={at={(0.9,0.9)}, anchor=north east, font=\small}
        ]
        \addplot[fill=blue!30, draw=blue!50] coordinates {({ASQA},61.38) ({ELI5},36.92) ({QAMPARI},18.46)};
        \addplot[fill=teal!50, draw=teal!70, xshift=-0.15em] coordinates {({ASQA},65.61) ({ELI5},41.15) ({QAMPARI},21.35)};

  \addlegendentry{Pre-filtered}
  \addlegendentry{Post-filtered}

      \end{axis}
    }
    }
    \end{tikzpicture}
    \caption{Ablation Study on Data Filtering.}
    \label{fig:ablation_data_filtering}
    \end{figure}

==> TMLR_Survey/Figure/Figure_Communication.tex <==
\definecolor{ublue}{RGB}{52,152,219}
\definecolor{ured}{RGB}{240,100,100}
\definecolor{uorange}{RGB}{247,175,89}
\definecolor{upurple}{RGB}{148,137,250}
\definecolor{pink1}{HTML}{FFF0F6}
\definecolor{pink2}{HTML}{FCC2D7}
\definecolor{pink3}{HTML}{FAA2CA}
% \definecolor{c1}{HTML}{FFD3AB}
% \definecolor{c2}{HTML}{FFEBDA}
% \definecolor{c3}{HTML}{FFFDFC}
% \definecolor{c4}{HTML}{E9F0FA}
% \definecolor{c5}{HTML}{DDE8F8}
% \definecolor{c6}{HTML}{EEF9E9}

\definecolor{c1}{HTML}{FFF0F5}
\definecolor{c2}{HTML}{F0E68C}
\definecolor{c3}{HTML}{D2EFB2}
\definecolor{c4}{HTML}{BFEFFF}

\definecolor{c5}{HTML}{A4D3EE}
\definecolor{c6}{HTML}{F0FFF0}

\hspace{-1.2cm} 
\begin{tikzpicture}
    \centering
    \scriptsize{
    \begin{axis}[
    at={(0,0)},
    ymajorgrids,
    % xmajorgrids,
    grid style=dashed,
    legend style={at={(0.2,1)}, anchor=south west},
    legend cell align={left},
    ybar,
    enlarge x limits=0.8,
    xtick align=inside,
    height=0.35\textwidth,
    width=0.5\textwidth,
    bar width=2.2em,
    xshift=-1.5em,
    nodes near coords,
    nodes near coords align={vertical},
    nodes near coords style={font=\tiny, scale=1,/pgf/number format/fixed, /pgf/number format/precision=1},
    every node near coord/.append style={
    /pgf/number format/.cd,
    fixed,
    fixed zerofill,
    precision=1
    },
    xlabel={},
    xmax=0,
    xmin=0,
    symbolic x coords={0},
    legend style={cells={align=left}},
    xtick=data,
    nodes near coords align={vertical},
    ymin=0,
    ymax=15,
    ytick={0,5,10,15},
    yticklabels={0,5,10,15},
    xticklabels={},
    xtick style={draw=none},
    ytick style={draw=none},
    % ylabel style={yshift=-3em},xlabel style={yshift=0.3em,align=center},
    yticklabel style={/pgf/number format/fixed,/pgf/number format/fixed},
    legend style={draw=none,
    line width=1pt,
    at={(0.5,1.0)},
    anchor=south},
    xtick=data,
    axis on top=false,
    ]
    \addplot[fill=c6,draw=gray, area legend] coordinates {(0,3.7)};
    \addplot[fill=c1, draw=gray, area legend] coordinates {(0,1.1)};
    \addplot[ fill=c2,draw=gray, area legend] coordinates {(0,3)};
    \addplot[ fill=c3,draw=gray, area legend] coordinates {(0,7)};
    \addplot[ fill=c4,draw=gray, area legend] coordinates {(0,8)};
    \addplot[ fill=c5,draw=gray, area legend] coordinates {(0,13)};
    \end{axis}
    }
    \node [rectangle,draw=gray,fill=c6,inner sep=2pt,minimum height=0.8em,minimum width=2.5em,font=\small,anchor=north,align=center,] (label1) at (1em,12em){};
    \node [rectangle,draw=gray,fill=c1,inner sep=2pt,minimum height=0.8em,minimum width=2.5em,font=\small,anchor=north,align=center,] (label2) at (1em,11em){};
    \node [rectangle,draw=gray,,fill=c2,inner sep=2pt,minimum height=0.8em,minimum width=2.5em,font=\small,anchor=north,align=center,] (label3) at (1em,10em){};
    \node [rectangle,draw=gray,,fill=c3,inner sep=2pt,minimum height=0.8em,minimum width=2.5em,font=\small,anchor=north,align=center,] (label4) at (1em,9em){};
    \node [rectangle,draw=gray,,fill=c4,inner sep=2pt,minimum height=0.8em,minimum width=2.5em,font=\small,anchor=north,align=center,] (label5) at (1em,8em){};
    \node [rectangle,draw=gray,,fill=c5,inner sep=2pt,minimum height=0.8em,minimum width=2.5em,font=\small,anchor=north,align=center,] (label6) at (1em,7em){};
    \node [align=center] (label1_1) at ([xshift=4.8em,yshift=-0.35em]label1.north){\tiny BERT};
    \node [align=center] (label1_2) at ([xshift=5em,yshift=-0.35em]label2.north){\tiny TinyLLaMA};
    \node [align=center] (label1_3) at ([xshift=5em,yshift=-0.35em]label3.north){\tiny LLaMA3-3B};
    \node [align=center] (label1_4) at ([xshift=5em,yshift=-0.35em]label4.north){\tiny LLaMA2-7B};
    \node [align=center] (label1_5) at ([xshift=5em,yshift=-0.35em]label5.north){\tiny LLaMA3-8B};
    \node [align=center] (label1_6) at ([xshift=5em,yshift=-0.35em]label6.north){\tiny LLaMA2-13B};
    
    \node [rotate=90]at (-4.8em,6.3em) {\footnotesize{Parameters (B)}};
\end{tikzpicture}



==> TMLR_Survey/Table/Table_Evaluation_datasets.tex <==
\begin{table}[!t]
\footnotesize
\centering
\renewcommand{\arraystretch}{1.1} 

\caption{Overview of general-domain evaluation benchmarks. Benchmarks specifically designed for \textit{long-context} (LC) evaluation are highlighted. For each benchmark, we summarize its primary evaluation objective and the main evaluation criteria.}

\label{tab_eva_benchmark}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule[1pt]
\midrule[0.5pt]

\textbf{Benchmark} & \textbf{Domain} & \textbf{Evaluation Objective} & \textbf{Main Evaluation Criteria} \\ 
\midrule[0.5pt]

\href{https://huggingface.co/datasets/cais/mmlu}{MMLU} & Gen. & Multitask understanding (57 subjects) & Multitask Accuracy \\

\href{https://huggingface.co/datasets/bigbench/bigbench}{BIG-bench} & Gen. & Advanced reasoning capabilities & Performance \& Calibration

\href{https://huggingface.co/datasets/drop}{DROP} & Gen. & Evaluate discrete reasoning over paragraphs & Exact match and F1 score \\

\href{https://github.com/apergo-ai/CRASS-data-set}{CRASS} & Gen. & Evaluate counterfactual reasoning ability in LLMs & Multiple-choice accuracy\\


\href{https://huggingface.co/datasets/ai2_arc}{ARC} & Gen. & Assess science reasoning at grade-school level & Multiple-choice accuracy \\


\href{https://huggingface.co/datasets/AGIEval/agieval}{AGIEval} & Gen. & Evaluate foundation models on human-centric standardized exam tasks & Multi-task accuracy across disciplines \\


\href{https://github.com/DAMO-NLP-SG/M3Exam}{M3Exam} & Gen. & Evaluate multilingual, multimodal, and multilevel reasoning across real exam questions & Multiple-choice accuracy \\

\href{https://github.com/mandyyyyii/scibench}{SCIBENCH} & Gen. & Evaluate college-level scientific problem-solving in math, physics, and chemistry & Open-ended accuracy and skill-specific error attribution \\

\href{https://github.com/lm-sys/FastChat}{Vicuna Evaluation} & Gen. & Evaluate instruction-following quality in chat settings & Human/GPT‑4 preference comparison accuracy \\

\href{https://github.com/lm-sys/FastChat/tree/main/mt-bench}{MT‑Bench} & Gen. & Evaluate multi‑turn conversational and instruction‑following capabilities & Winrate judged by GPT-4 \\


\href{https://github.com/tatsu-lab/alpaca_eval}{AlpacaEval} & Gen. & Evaluate instruction-following performance via LLM-based auto-annotation & Length-controlled win rate correlated with human preference accuracy \\

\href{https://github.com/lm-sys/FastChat/blob/main/docs/arena.md}{Chatbot Arena} & Gen. & Evaluate LLMs via human-voted battles using Elo rating & Elo score and head-to-head win rate \\

\href{https://github.com/YiXiangzhong/PandaLM}{PandaLM} & Gen. & Evaluate instruction-following quality and hyperparameter impact & Winrate judged by PandaLM \\ 


\href{https://huggingface.co/datasets/rowanz/hellaswag}{HellaSwag} & Gen. & Evaluate commonsense inference by selecting the most plausible continuation & Multiple-choice accuracy\\


\href{https://huggingface.co/datasets/truthful_qa}{TruthfulQA} & Gen. & Evaluate LLM truthfulness and avoidance of imitative falsehoods & Truthfulness rate and MC accuracy \\



\href{https://huggingface.co/datasets/lupantech/scienceqa}{ScienceQA} & Gen. & Evaluate multimodal scientific reasoning and explanation generation & Multiple-choice accuracy and explanation quality \\

\href{https://github.com/FranxYao/chain-of-thought-hub}{Chain-of-Thought Hub} & Gen. & Evaluate LLMs' multi-step reasoning across diverse domains using CoT prompting & Few-shot CoT accuracy\\

\href{https://github.com/DeepReasoning/NeuLR}{NeuLR} & Gen. & Evaluate deductive, inductive, and abductive reasoning capabilities of LLMs & Multi-dimensional evaluation (e.g., accuracy, self-awareness) \\

\href{https://github.com/hyintell/alcuna}{ALCUNA} & Gen. & Evaluate LLMs’ ability to comprehend and reason over novel knowledge & Accuracy on 84,351 queries\\

\href{https://github.com/LeapLabTHU/LMExam}{LMExamQA} & Gen. & Evaluate LLMs' performance across knowledge recall, understanding, and analysis & Accuracy on 10,090 questions\\

\href{https://github.com/minjechoi/SOCKET}{SocKET} & Gen. & Evaluate LLMs’ sociability and understanding of social knowledge & Accuracy and other metrics\\

\href{https://arxiv.org/abs/2309.11737}{Choice-75} & Gen. & Evaluate LLMs’ decision reasoning ability within scripted scenarios & Accuracy on binary multiple-choice questions \\

\href{https://github.com/stanford-crfm/helm}{HELM} & Gen. & Evaluate LMs via multi‑metric scenarios & Composite performance ranking (normalized scores across metrics) \\

\href{https://github.com/bentoml/openllm-benchmark}{OpenLLM} & Gen. & Evaluate open‑style reasoning across multiple benchmarks & Normalized accuracy aggregate across tasks \\

\midrule[0.5pt]


\href{https://github.com/lifan-yuan/OOD_NLP}{BOSS} & Gen. & Evaluate out-of-distribution robustness across NLP tasks & OOD accuracy drop and ID–OOD performance correlation \\

\href{https://github.com/YangLinyi/GLUE-X}{GLUE‑X} & Gen. & Evaluate out‑of‑distribution robustness & Average OOD accuracy drop relative to ID performance \\

\href{https://github.com/microsoft/promptbench}{PromptBench} & Gen. & Evaluate robustness, prompt-engineering and dynamic evaluation capabilities & Adversarial success rate, robustness, prompt-variant performance \\

\href{https://github.com/facebookresearch/dynabench}{DynaBench} & Gen. & Evaluate robustness via dynamic, human-in-loop adversarial data collection & Model error rate on human-crafted challenge examples \\

\href{https://github.com/THU-KEG/KoLA}{KoLA} & Gen. & Evaluate world knowledge across 19 evolving tasks & self-contrast calibration \\

\href{https://github.com/Abbey4799/CELLO}{CELLO} & Gen. & Evaluate following complex, real-world instructions with multiple constraints & Multi-criteria compliance rate judged by automated metrics \\


\href{https://github.com/UMass-Meta-LLM-Eval/llm_eval}{LLMEval} & Gen. & Evaluate LLM evaluators’ ability to assess instruction-following quality & Meta-evaluator accuracy\\

\midrule[0.5pt]


\href{https://github.com/MikeGu721/XiezhiBenchmark}{Xiezhi} & Gen. & Evaluate holistic domain knowledge across 516 disciplines & Mean Reciprocal Rank (MRR) \\

\href{https://github.com/hkust-nlp/ceval}{C‑Eval} & Gen. & Evaluate Chinese domain knowledge and reasoning across 52 disciplines & Multiple‑choice accuracy \\

\href{https://github.com/LianjiaTech/BELLE/tree/main/eval}{BELLE-eval} & Gen. & Evaluate Chinese instruction-following and multi-skill capabilities & GPT‑4 adjudicated win-rate and per‑task quality scores \\

\href{https://github.com/CLUEbenchmark/SuperCLUE}{SuperCLUE} & Gen. & Evaluate Chinese instruction-following with human preference alignment & GPT‑4 adjudicated win-rate and Elo scores \\  

\href{https://github.com/tjunlp-lab/M3KE}{M3KE} & Gen. & Evaluate Chinese LLMs' knowledge across 71 disciplines and 4 education levels & Multitask accuracy in zero- and few-shot settings \\

\href{https://github.com/ictnlp/BayLing}{BayLing-80} & Gen. & Evaluate cross-lingual  and conversational capabilities & GPT-4 adjudicated win-rate\\

\href{https://huggingface.co/datasets/Besteasy/MMCU}{MMCU} & Gen. & Evaluate multitask Chinese understanding across different domains & Multitask accuracy (zero-/few-shot) \\


\href{https://github.com/jizijing/C-CLUE}{C‑CLUE} & Gen. & Evaluate classical Chinese NER and relation extraction capabilities & Weighted F1 score for NER and RE tasks \\



\midrule[0.5pt]

\href{https://huggingface.co/datasets/THUDM/LongBench}{LongBench} & Gen. (LC) & Evaluate bilingual long-context understanding across multiple real-world tasks & Accuracy and generation quality \\

\href{https://github.com/OpenLMLab/LEval}{L-Eval} & Gen. (LC) & Evaluate long-context reasoning and task performance over documents up to 60K tokens & Multi-metric assessment \\

\href{https://github.com/OpenBMB/InfiniteBench}{InfinityBench} & Gen. (LC) & Evaluate long-context understanding across tasks up to 2M tokens in length & Accuracy and task-specific metrics \\

\href{https://github.com/Hambaobao/Marathon}{Marathon} & Gen. (LC) & Evaluate long-context understanding across multi-domain and multi-task settings & Accuracy, F1, ROUGE-L, EM across tasks and context lengths \\


\href{https://github.com/DachengLi1/LongChat}{LongEval} & Gen. (LC) & Evaluate LLMs' effectiveness in long-context retrieval tasks & Accuracy in broad-topic and fine-grained passage retrieval\\


\href{https://github.com/booydar/babilong}{BABILong} & Gen. (LC) & Evaluate long-context reasoning in haystack-like settings & Accuracy on long-context reasoning tasks \\


\href{https://github.com/Phospheneser/DetectiveQA}{DetectiveQA} & Gen. (LC) & Evaluate long-context reasoning through detective novel comprehension & Instruction-following accuracy and winrate judged by PandaLM \\



\href{https://github.com/marzenakrp/nocha}{NoCha} & Gen. (LC) & Evaluate narrative comprehension and long-range coreference resolution in literary texts & Exact match and accuracy \\


\href{https://github.com/MozerWang/Loong}{Loong} & Gen. (LC) & Evaluate LLMs' ability to perform multi-document reasoning and extended-context question answering & Answer accuracy, context utilization rate, and document coverage score \\


\href{https://github.com/Zhihan72/TCELongBench}{TCELongBench} & Gen. (LC) & Evaluate temporal reasoning over complex, long event narratives & Temporal event ordering accuracy and event query answering accuracy \\




\href{https://github.com/ameliadai/DENIAHL}{DENIAHL} & Gen. (LC) & Evaluate the influence of in-context features on LLMs’ needle-in-a-haystack abilities & Accuracy on long-context retrieval and reasoning tasks \\

\href{https://arxiv.org/abs/2410.10813}{LongMemEval} & Gen. (LC) & Benchmark LLMs' ability to retain and utilize long-term interactive memory across dialogue sessions & Memory retention accuracy, retrieval success rate, and context utilization score \\

\href{https://arxiv.org/abs/2401.13619}{Long2RAG} & Gen. (LC) & Evaluate long-form generation and retrieval grounding under extended input lengths & Key point recall, LLM-based coherence, factuality, and answer relevance \\


\href{https://github.com/ZetangForward/L-CITEEVAL}{L-CiteEval} & Gen. (LC) & Evaluate LLMs' ability to utilize citations and contextual evidence & Citation recall, LLM-based factuality and faithfulness scoring \\


\href{https://github.com/sheldonwu0327/lif-bench-2024}{LIFBENCH} & Gen. (LC) & Evaluate instruction-following performance and robustness in long-context scenarios & Instruction-following accuracy and response stability \\

\href{https://arxiv.org/abs/2310.00991}{LongReason} & Gen. (LC) & Evaluate long-context reasoning via synthetic context expansion & Instruction-following accuracy and reasoning correctness\\

\href{https://github.com/RUCAIBox/BAMBOO}{BAMBOO} & Gen. (LC) & Evaluate long-text modeling capacity across diverse real-world tasks & Instruction-following accuracy and winrate judged by PandaLM  \\


\href{https://arxiv.org/abs/2312.06318}{ETHIC} & Gen. (LC) & Evaluate instruction-following on long-context tasks with high information coverage & Exact match, F1, and consistency/completeness\\

\href{https://github.com/bigai-nlco/LooGLE}{LooGLE} & Gen. (LC) & Evaluate LLMs’ ability to understand and reason over long contexts & Accuracy on inputs averaging 20K words \\

\href{https://github.com/megagonlabs/llm-longeval}{HELMET} & Gen. (LC) & Evaluate instruction-following, retrieval, reasoning, summarization, and long-context understanding & Task-specific automatic metrics and human evaluation\\


\href{https://arxiv.org/abs/2405.06416}{HoloBench} & Gen. (LC) & Evaluate LLMs’ holistic reasoning ability over database-style textual inputs & Execution accuracy and reasoning consistency on DB-style tasks \\


\href{https://arxiv.org/abs/2402.05829}{LOFT} & Gen. (LC) & Evaluate whether long-context LLMs can replace retrieval-augmented methods in complex tasks & EM/F1, SQL exec. accuracy, LLM-based factuality and reasoning coherence \\




\href{https://github.com/infinigence/LVEval}{Lv-Eval} & Gen. (LC) & Evaluate long-context comprehension across five input length levels (up to 256k tokens) & Exact match, ROUGE-L, LLM-based factuality and relevance scoring \\

\href{https://arxiv.org/abs/2404.01237}{ManyICLBench} & Gen. (LC) & Evaluate many-shot in-context learning capabilities under extended context lengths & Average accuracy across tasks under different context lengths\\


\href{https://arxiv.org/abs/2403.05331}{ZeroSCROLLS} & Gen. (LC) & Evaluate zero-shot inference capabilities of LLMs on diverse long-text tasks & Accuracy on inputs averaging 10K words \\


\href{https://arxiv.org/abs/2403.11935}{LongICLBench} & Gen. (LC) & Evaluate long-context LLMs' capability in in-context learning under extended input lengths & Winrate judged by PandaLM \\


\href{https://arxiv.org/abs/2408.02439}{LIBRA} & Gen. (LC) & Evaluate long-context understanding and instruction-following in Russian & Accuracy, BLEU, LLM-based faithfulness and coherence scoring \\




\midrule[0.5pt]
\bottomrule[1pt]
\end{tabular}
}
\vspace{-3mm}
\end{table}


==> TMLR_Survey/Table/Table_Finetune_dataset.tex <==
\begin{table}[!t]
\footnotesize
\centering
\caption{A summary of representative \textbf{instruction fine-tuning datasets}. The construction methods are categorized into three types: human construct, which refers to datasets manually written or annotated by humans; model construct, which refers to data generated by prompting LLMs; and synthetic, which refers to data produced through rule-based or programmatic generation. The datasets span key domains such as general language understanding, finance, medicine, code, math, and law.}
\label{tab_finetune_dataset}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule[1pt]
\midrule[0.5pt]

\textbf{Dataset}& \textbf{Language} &\textbf{Construction Method} & \textbf{Domain} & \textbf{Description} \\ 

\midrule[0.5pt]
\href{https://huggingface.co/datasets/tatsu-lab/alpaca_farm}{Alpaca} & English & Model Construct & General & 
Generated by Text-Davinci-003 with Alpaca-style instruction prompts.\\

\href{https://huggingface.co/datasets/vicgalle/alpaca-gpt4}{Alpaca-GPT4} & English & Model Construct & General & Generated by GPT-4 based on Alpaca prompts with more nuanced multi-turn instructions.\\

\href{https://huggingface.co/datasets/yizhongw/self_instruct}{Self-Instruct} & English & Human + Model Construct & General & Dataset from seed instructions using GPT-3 for improving model generalization.\\


\href{https://huggingface.co/datasets/HuggingFaceH4/ultrachat_200k}{UltraChat 200k} & English & Model Construct & General & High-quality multi-turn dialogue dataset filtered from UltraChat.\\


\href{https://huggingface.co/datasets/Open-Orca/OpenOrca}{OpenOrca} & English & Model Construct & General &  Dataset of $\sim$ 
4.2M GPT-3.5/4 augmented FLAN examples for instruction following.\\


\href{https://huggingface.co/datasets/anon8231489123/ShareGPT_Vicuna_unfiltered}{ShareGPT90K} & English & Model Construct & General & 
Multi-turn dialogue dataset of 90K samples derived from ShareGPT for instruction following.\\

\href{https://huggingface.co/datasets/WizardLMTeam/WizardLM_evol_instruct_V2_196k}{WizardLM Evol-Instruct V2 196k} & English & Model Construct & General & Dataset of 196K samples generated via Evol-Instruct method.\\

\href{https://huggingface.co/datasets/databricks/databricks-dolly-15k}{Databricks Dolly 15K} & English & Human Construct & General & Dataset of 15K human-generated prompt-response pairs across diverse tasks.\\


\href{https://huggingface.co/datasets/linkanjarad/baize-chat-data}{Baize} & English & Model Construct & General & Instruction-following dialogues generated by prompting ChatGPT with user-centric queries.\\

\href{https://huggingface.co/datasets/openchat/ultrachat-sharegpt}{OpenChat} & English & Model Construct & General & Instruction-following dialogues generated using open LLMs for multi-turn alignment.\\


\href{https://huggingface.co/datasets/SirNeural/flan_v2}{Flan-v2} & English & Model Construct & General & Dataset combining Flan, P3, Super-Natural Instructions, Chain-of-thought, and Dialog tasks.\\

\href{https://huggingface.co/datasets/BelleGroup/train_0.5M_CN}{BELLE-train-0.5M-CN} & Chinese & Human + Model Construct & General & Dataset of 519K Chinese samples for instruction following.\\

\href{https://huggingface.co/datasets/BelleGroup/train_1M_CN}{BELLE-train-1M-CN} & Chinese & Human + Model Construct & General & Dataset of 917K Chinese samples for instruction following.\\


\href{https://huggingface.co/datasets/BelleGroup/train_2M_CN}{BELLE-train-2M-CN} & Chinese & Human + Model Construct & General & Dataset of 2M Chinese samples for instruction following.\\


\href{https://huggingface.co/datasets/YeungNLP/firefly-train-1.1M}{Firefly-train-1.1M} & Chinese & Human Construct & General & Dataset of 1.65M Chinese samples across 23 tasks with human-written instruction templates.\\


\href{https://huggingface.co/datasets/silk-road/Wizard-LM-Chinese-instruct-evol}{Wizard-LM-Chinese-instruct-evol} & Chinese & Human + Model Construct & General & 
Dataset of 70K samples translated from WizardLM to Chinese with GPT-generated responses.\\

\href{https://huggingface.co/datasets/Hello-SimpleAI/HC3-Chinese}{HC3-Chinese} & Chinese & Human + Model Construct & General & 
Chinese Human-ChatGPT QA pairs across multiple domains.\\



\href{https://huggingface.co/datasets/Hello-SimpleAI/HC3}{HC3} & English / Chinese & Human + Model Construct & General & 
Human-ChatGPT QA pairs across multiple domains.\\

\href{https://huggingface.co/datasets/anon8231489123/ShareGPT_Vicuna_unfiltered}{ShareGPT-Chinese-English-90k} & English / Chinese & Model Construct & General & Bilingual human-machine QA dataset of 90K real user queries in Chinese and English.\\


\midrule[0.5pt]

\href{https://huggingface.co/datasets/FinGPT/fingpt-finred}{FinGPT} & English & Human + Model Construct & Finance & Instruction tuning data for financial tasks.\\

\href{https://huggingface.co/datasets/Josephgflowers/Finance-Instruct-500k}{Finance-Instruct-500k} & English & Human + Model Construct & Finance & 
Large-scale instruction tuning dataset for financial tasks.\\

\href{https://huggingface.co/datasets/gbharti/finance-alpaca}{Finance-Alpaca} & English & Human + Model Construct & Finance & 
Instruction tuning dataset combining Alpaca and FiQA.\\

% Instruct-FinGPT & English & Human + Model Construct & Finance & Human and GPT-generated financial prompts and answers.\\

\href{https://huggingface.co/datasets/takala/financial_phrasebank}{Financial PhraseBank} & English & Human Construct & Finance & Manually annotated financial news sentences for sentiment classification.\\

\href{https://huggingface.co/datasets/bwzheng2010/yahoo-finance-data}{Yahoo-Finance-Data} & English & Human Construct & Finance & Financial dataset including estimates, statements, and historical prices from Yahoo Finance.\\

\href{https://huggingface.co/datasets/virattt/financial-qa-10K}{Financial-QA-10K} & English &  Model Construct & Finance & Contextual QA dataset for financial question answering and retrieval tasks.\\

\href{https://huggingface.co/datasets/nickmuchi/financial-classification}{Financial-Classification} & English & Human  Construct & Finance & 
Dataset combining Financial PhraseBank and Kaggle financial texts.\\

\href{https://huggingface.co/datasets/zeroshot/twitter-financial-news-topic}{Twitter-Financial-News-Topic} & English & Human Construct & Finance & 
Annotated tweets for multi-class financial topic classification tasks.\\

\href{https://huggingface.co/datasets/ashraq/financial-news-articles}{Financial-News-Articles} & English & Human Construct & Finance & Financial news articles for text classification and sentiment analysis tasks.\\


\href{https://huggingface.co/datasets/BeIR/fiqa}{FiQA} & English & Human Construct & Finance & QA dataset from financial texts and forums covering finance topics.\\

\href{https://huggingface.co/datasets/lamini/earnings-calls-qa}{Earnings-Call} & English & Human Construct & Finance & QA pairs from CEO/CFO earnings calls for financial reasoning.\\

\href{https://github.com/shun-zheng/Doc2EDAG}{Doc2EDAG} & Chinese & Human Construct & Finance & Financial reports annotated for event graph extraction and structuring.\\

\href{https://huggingface.co/datasets/gretelai/synthetic_pii_finance_multilingual}{Synthetic-PII-Finance-Multilingual} & Multilingual & Synthetic & Finance & Financial documents with labeled PII for NER and privacy-preserving model training.\\


\midrule[0.5pt]

\href{https://huggingface.co/datasets/LinhDuong/chatdoctor-200k}{ChatDoctor-200K} & English & Human + Model Construct & Medical & Instruction tuning dataset for medical QA and dialogue generation.\\

\href{https://huggingface.co/datasets/lavita/ChatDoctor-HealthCareMagic-100k}{ChatDoctor-HealthCareMagic-100k} & English & Human Construct & Medical & 
Real-world doctor-patient conversations.\\


\href{https://huggingface.co/datasets/medalpaca/medical_meadow_cord19}{Medical Meadow CORD-19} & English & Human  Construct & Medical & Instruction tuning dataset for medical literature summarization based on CORD-19.\\

\href{https://huggingface.co/datasets/medalpaca/medical_meadow_medqa}{Medical Meadow MedQA} & English & Human Construct & Medical & 
Multiple-choice medical QA dataset derived from professional medical board exams.\\

\href{https://huggingface.co/datasets/wangrongsheng/HealthCareMagic-100k-en}{HealthCareMagic-100k-en} & English & Human Construct & Medical & Real doctor-patient consultations for instruction tuning.\\


\href{https://huggingface.co/datasets/michaelwzhu/ChatMed_Consult_Dataset}{ChatMed-Consult-Dataset} & Chinese & Human + Model Construct & Medical & Instruction tuning dataset of Chinese medical consultations for QA and dialogue generation.\\

\href{https://github.com/SupritYoung/Zhongjing}{CMtMedQA} & Chinese & Human Construct & Medical & Multi-turn medical QA dataset with real doctor-patient conversations.\\

\href{https://huggingface.co/datasets/Flmc/DISC-Med-SFT}{DISC-Med-SFT} & Chinese & Human + Model Construct & Medical & Instruction tuning dataset combining real-world dialogues and knowledge graph QA pairs.\\

\href{https://huggingface.co/datasets/FreedomIntelligence/huatuo26M-testdatasets}{Huatuo-26M} & Chinese & Human  Construct & Medical & Structured QA pairs extracted from medical encyclopedias and articles.\\

\href{https://huggingface.co/datasets/FreedomIntelligence/Huatuo26M-Lite}{Huatuo26M-Lite} & Chinese & Human + Model Construct & Medical & 
Refined subset of Huatuo-26M with ChatGPT-rewritten answers.\\

\href{https://huggingface.co/datasets/michaelwzhu/ShenNong_TCM_Dataset}{ShenNong-TCM-Dataset} & Chinese & Human + Model Construct & Medical & QA pairs generated via entity-centric self-instruct from a TCM knowledge graph.\\


\href{https://huggingface.co/datasets/FreedomIntelligence/HuatuoGPT-sft-data-v1}{HuatuoGPT-sft-data-v1} & Chinese & Human + Model Construct & Medical & 
Instruction tuning dataset combining ChatGPT-generated and real doctor-patient dialogues.\\

\href{https://huggingface.co/datasets/bigbio/meddialog}{MedDialog} & English / Chinese & Human Construct & Medical & 
Large-scale doctor-patient dialogues for medical QA and dialogue generation.\\

\midrule[0.5pt]

\href{https://huggingface.co/datasets/sahil2801/CodeAlpaca-20k}{CodeAlpaca} & English & Model Construct & Code & GPT-generated code instruction-following dataset based on the Alpaca style.\\

\href{https://huggingface.co/datasets/iamtarun/code_instructions_120k_alpaca}{Code Instructions 120k Alpaca} & English & Human + Model Construct & Code & Instruction tuning dataset for code generation with prompts in alpaca style.\\

\href{https://huggingface.co/datasets/deepmind/code_contests}{CodeContests} & English & Human Construct & Code & Dataset from competitive programming platforms, designed for program synthesis and reasoning.\\

\href{https://huggingface.co/datasets/bigcode/commitpackft}{CommitPackFT} & English & Human Construct & Code & Filtered dataset of GitHub commits with high-quality messages for code generation tasks.\\

\href{https://github.com/OpenBMB/ToolBench}{ToolBench} & English & Human + Model Construct & Code & Instruction tuning dataset for multi-tool API usage scenarios.\\


\href{https://huggingface.co/datasets/codeparrot/codeparrot-clean}{CodeParrot-Clean} & English & Human Construct & Code & 
Deduplicated and filtered dataset of Python files from GitHub for code generation.\\

\href{https://huggingface.co/datasets/bigcode/the-stack-v2-dedup}{The Stack v2 Dedup} & English & Human Construct & Code & 
Large-scale deduplicated dataset of source code from 600+ programming languages.\\

\href{https://huggingface.co/datasets/irds/codesearchnet}{CodeSearchNet} & English & Human Construct & Code & 
Code-language pairs for retrieval and semantic search across six programming languages.\\

\href{https://huggingface.co/datasets/open-r1/codeforces-cots}{CodeForces-CoTs} & English & Human + Model Construct & Code & A dataset consists of 10k CodeForces problems with reasoning traces generated by DeepSeek R1. \\

\href{https://huggingface.co/datasets/google/code_x_glue_cc_code_refinement}{CodeXGLUE Code Refinement} & English & Human Construct & Code & Dataset of buggy and fixed Java functions for code refinement.\\



\midrule[0.5pt]

\href{https://huggingface.co/datasets/openai/gsm8k}{GSM8K} & English & Human Construct & Math &
A dataset of 8.5k grade school-level arithmetic word problems with detailed step-by-step solutions.\\

\href{https://huggingface.co/datasets/ankner/gsm8k-CoT}{CoT-GSM8k} & English & Human + Model Construct & Math & 
Extended version of GSM8K with chain-of-thought reasoning steps.\\


% MathInstruct & English & Model Construct & Math & GPT-generated instruction-following dataset for algebra, geometry, and logical math reasoning.\\

\href{https://huggingface.co/datasets/TIGER-Lab/MathInstruct}{MathInstruct} & English & Human + Model Construct & Math & Dataset combining CoT and program-of-thought rationales across diverse mathematical fields.\\


\href{https://huggingface.co/datasets/meta-math/MetaMathQA}{MetaMathQA} & English & Human + Model Construct & Math & Multi-perspective question augmentations from GSM8K and MATH.\\

\href{https://huggingface.co/datasets/open-r1/OpenR1-Math-220k}{OpenR1-Math-220k} & English & Human + Model Construct & Math & Dataset of 220k math problems with multiple reasoning traces generated by DeepSeek R1.\\

\href{https://huggingface.co/datasets/hendrycks/competition_math}{Hendrycks MATH Benchmark} & English & Human Construct & Math & 
Dataset of 12.5K high school competition math problems with step-by-step solutions.\\

\href{https://huggingface.co/datasets/deepmind/math_dataset}{DeepMind Mathematics Dataset} & English & Synthetic & Math & Dataset of algorithmically generated math problems across various topics.\\


\href{https://huggingface.co/datasets/nvidia/OpenMathInstruct-1}{OpenMathInstruct-1} & English & Human + Model Construct & Math & Dataset of 1.8M math problems with code-interpreter solutions generated by Mixtral-8x7B.\\

\href{https://huggingface.co/datasets/microsoft/orca-math-word-problems-200k}{Orca-Math Word Problems 200k} & English & Synthetic & Math & Synthetic dataset of 200K grade school math word problems with GPT-4 Turbo solutions.\\

\href{https://huggingface.co/datasets/BytedTsinghua-SIA/DAPO-Math-17k}{DAPO-Math-17k} & English & Human + Model Construct & Math & Dataset of 17K diverse math problems for mathematical reasoning.\\

\href{https://huggingface.co/datasets/SynthLabsAI/Big-Math-RL-Verified}{Big-Math-RL-Verified} & English & Human + Model Construct & Math & Dataset of 251K math problems with verifiable answers, curated for reinforcement learning.\\

\href{https://huggingface.co/datasets/BelleGroup/school_math_0.25M}{BELLE-math-zh} & Chinese & Human + Model Construct & Math & Dataset of Chinese elementary school math problems with step-by-step solutions.\\

\href{https://huggingface.co/datasets/ALmonster/MathInstruct-Chinese}{MathInstruct-Chinese} & Chinese & Model Construct & Math & Chinese version of MathInstruct; contains instruction-style math problems in Chinese.\\

\midrule[0.5pt]

\href{https://huggingface.co/datasets/dzunggg/legal-qa-v1}{Legal-QA-v1} & English & Human Construct & Law & Dataset of 3.7K legal question-answer pairs sourced from legal forums.\\

\href{https://huggingface.co/datasets/pile-of-law/pile-of-law}{Pile of Law} & English & Human Construct & Law & Dataset for legal-domain tasks.\\


\href{https://huggingface.co/datasets/theatticusproject/cuad}{CUAD} & English & Human Construct & Law & Expert-annotated dataset of 26K legal contract question-answer pairs across 41 clause categories.\\

\href{https://huggingface.co/datasets/coastalcph/lex_glue:ledgar}{LEDGAR} & English & Human Construct & Law &
Dataset of 1.45M contract clauses labeled by legal experts.\\


\href{https://huggingface.co/datasets/ShengbinYue/DISC-Law-SFT}{DISC-Law-SFT} & Chinese & Human + Model Construct & Law & Comprehensive instruction tuning dataset covering diverse legal tasks.\\

\href{https://huggingface.co/datasets/sentence-transformers/law-gpt}{Law-GPT-zh} & Chinese & Human Construct & Law & Dataset of legal sentence pairs for training sentence embedding models in legal domain.\\

\href{https://huggingface.co/datasets/Dusker/lawyer-llama}{Lawyer LLaMA Data} & Chinese & Human + Model Construct & Law & Dataset for Chinese legal tasks including legal consultation and bar exam question answering.\\

\midrule[0.5pt]
\bottomrule[1pt]
\end{tabular}
}
\end{table}

==> TMLR_Survey/Table/Table_adapter_multidomain.tex <==
\begin{table}[!t]
\small
\centering
\caption{\textbf{Multi-domain adapter tuning in federated fine-tuning.}}
\label{Adapter_muldomain_table}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Method}}& \multicolumn{4}{c}{\textbf{Challenge}}  \\  

\cmidrule{2-5}

& \textbf{Communication} & \textbf{Non-IID} & \textbf{Memory} & \textbf{Computation}  \\ 

\midrule[1pt]
{Fed-MNMT~\citep{liu2023communication}}&\hlr{\xmark}&\hlg{\tmark{}}&\hlr{\xmark}&\hlr{\xmark}\\
{AdaFedSelecKD~\citep{feng2024adapter}}&\hlr{\xmark}&\hlg{\tmark{}}&\hlr{\xmark}&\hlr{\xmark}\\
{FedDAT~\citep{chen2024feddat}}&\hlr{\xmark}&\hlg{\tmark{}}&\hlr{\xmark}&\hlr{\xmark}\\
\bottomrule[1pt]
\end{tabular}
}
\end{table}

==> TMLR_Survey/Table/Table_adapter_personalized.tex <==
\begin{table}[!t]
\small
\centering
\caption{\textbf{Personalized adapter tuning in federated fine-tuning.}}
\label{Adapter_person_table}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Method}}& \multicolumn{4}{c}{\textbf{Challenge}}  \\  
\cmidrule{2-5}
& \textbf{Communication} & \textbf{Non-IID} & \textbf{Memory} & \textbf{Computation} \\ 

\midrule[1pt]
{C2A~\citep{kim2023client}}&\hlr{\xmark}&\hlg{\tmark{}}&\hlr{\xmark}&\hlr{\xmark}\\
{FedCLIP~\citep{lu2023fedclip}}&\hlr{\xmark}&\hlg{\tmark{}}&\hlr{\xmark}&\hlr{\xmark}\\

\bottomrule[1pt]
\end{tabular}
}

\end{table}

==> TMLR_Survey/Table/Table_evaluation_domain_specific.tex <==
\begin{table}[!t]
\footnotesize
\centering
\renewcommand{\arraystretch}{1.1}  
\caption{Overview of evaluation benchmarks across five specialized domains: \textbf{finance}, \textbf{medicine}, \textbf{code}, \textbf{math}, and \textbf{law}. The table summarizes representative benchmarks along with their primary evaluation objectives, target domains, and main evaluation criteria.}

\label{tab_eva_benchmark_domain}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule[1pt]
\midrule[0.5pt]

\textbf{Benchmark} & \textbf{Domain} & \textbf{Evaluation Objective} & \textbf{Main Evaluation Criteria} \\ 
\midrule[0.5pt]

\href{https://huggingface.co/datasets/TheFinAI/finben-finer-ord}{FinBen} & Finance & Evaluate holistic financial capabilities across 24 tasks & Automatic metrics, agent/RAG performance, and human expert assessment \\


\href{https://huggingface.co/ICE-PIXIU}{PIXIU} & Finance & Evaluate LLMs across multiple financial NLP tasks & Sentiment accuracy, QA accuracy, stock prediction F1 \\

\href{https://huggingface.co/datasets/SALT-NLP/FLUE-FiQA}{FLUE} & Finance & Evaluate diverse financial NLP competencies & Accuracy, F1, nDCG\\

\href{https://github.com/ssymmetry/BBT-FinCUGE-Applications}{BBF-CFLEB} & Finance & Evaluate LLMs on Chinese financial language understanding and generation across six task types & Rouge, F1, and accuracy\\


\href{https://cfinbench.github.io}{CFinBench} & Finance & Evaluate Chinese financial knowledge across subjects, certifications, practice, and legal compliance & Accuracy across single-choice, multiple-choice, and judgment questions \\

\href{https://arxiv.org/abs/2404.19063}{SuperCLUEFin} & Finance & Evaluate Chinese financial assistant capabilities & Win-rate and multi-criteria performance \\

\href{https://github.com/YY0649/ICE-PIXIU}{ICE‑PIXIU} & Finance & Evaluate bilingual (Chinese–English) financial reasoning and analysis capabilities & Task-specific accuracy and bilingual win‑rate \\

\href{https://arxiv.org/abs/2402.07405}{FLARE‑ES} & Finance & Evaluate bilingual Spanish–English financial reasoning & Task‑specific accuracy and cross‑lingual transfer win‑rate \\

\href{https://github.com/patronus-ai/financebench}{FinanceBench} & Finance & Evaluate financial open-book QA using real-world company-related questions & Factual correctness and evidence alignment\\


\href{https://huggingface.co/datasets/gtfintechlab/finer-ord}{FiNER‑ORD} & Finance & Evaluate financial NER capability in financial texts & Entity F1\\

\href{https://huggingface.co/datasets/FinGPT/fingpt-finred}{FinRED} & Finance & Evaluate financial relation extraction performance on news and earnings transcripts & F1, Entity F1\\

\href{https://huggingface.co/datasets/czyssrs/FinQA}{FinQA} & Finance & Evaluate multi-step numerical reasoning over financial reports with structured evidence & EM Accuracy\\

\href{https://huggingface.co/datasets/kensho/bizbench}{BizBench} & Finance & Evaluate quantitative reasoning on realistic financial problems & Numeric EM, code execution pass rate, QA accuracy \\


\href{https://huggingface.co/datasets/yinzhu-quan/econ_logic_qa}{EconLogicQA} & Finance & Evaluate economic sequential reasoning across multi-event scenarios & Multiple-choice accuracy \\

\href{https://github.com/SUFE-AIFLM-Lab/FinEval}{FinEval} & Finance & Evaluate Chinese financial domain knowledge and reasoning & Multiple-choice accuracy and task-level weighted scores \\


\href{https://github.com/TongjiFinLab/CFBenchmark}{CFBenchmark} & Finance & Evaluate Chinese financial assistant capabilities & Win-rate and task-specific metrics \\

\href{https://github.com/ssymmetry/BBT-FinCUGE-Applications}{BBT-Fin} & Finance & Evaluate Chinese financial language understanding and generation & Accuracy, F1, ROUGE \\


\href{https://github.com/pfnet-research/japanese-lm-fin-harness}{Hirano} & Finance & Evaluate Japanese financial language understanding & Multiple-choice accuracy and macro-F1 scores \\  


\href{https://huggingface.co/datasets/awinml/MultiFin}{MultiFin} & Finance & Evaluate multilingual financial topic classification & F1, Multi-class accuracy \\ 


\href{https://huggingface.co/datasets/kensho/DocFinQA}{DocFinQA} & Finance (long-context) & Evaluate long-context financial reasoning over documents like financial reports & EM and F1 for multi-step answer prediction, and reasoning accuracy \\

\href{https://huggingface.co/datasets/GPS-Lab/FinTextQA}{FinTextQA} & Finance (long-context) & Evaluate long-form financial question answering with long textual context & Answer accuracy, BLEU, and ROUGE \\



\midrule

\href{https://github.com/CBLUEbenchmark/CBLUE}{CBLUE} & Medical & Evaluate Chinese biomedical language understanding across multiple clinical and QA tasks & Accuracy, F1-score, and macro-average metrics across subtasks \\

\href{https://huggingface.co/datasets/Juvenilecris/CHIP2023-PromptCBLUE-peft}{PromptCBLUE} & Medical & Evaluate LLMs on prompt-based generation across 16 Chinese medical NLP tasks & Accuracy, BLEU, and ROUGE scores \\


\href{https://huggingface.co/datasets/FreedomIntelligence/CMB}{CMB} & Medical & Evaluate comprehensive Chinese medical knowledge via exam-style QA and clinical diagnosis tasks & Accuracy, expert grading, and model-based evaluation \\

\href{https://huggingface.co/datasets/FreedomIntelligence/huatuo26M-testdatasets}{HuaTuo26M-test} & Medical & Evaluate Chinese medical knowledge and QA ability using real-world clinical queries & Accuracy and relevance\\


\href{https://huggingface.co/datasets/fzkuji/CMExam}{CMExam} & Medical & Evaluate LLMs on Chinese medical licensing exam QA with fine-grained clinical annotations & Accuracy, weighted F1 score, and expert-judged reasoning quality \\


\href{https://www.nature.com/articles/s41591-024-03423-7}{MultiMedQA} & Medical & Evaluate LLMs’ clinical knowledge via multiple-choice and open-ended medical QA tasks & Expert-rated helpfulness, factuality, and safety \\


\href{https://github.com/CMKRG/QiZhenGPT}{QiZhenGPT eval} & Medical & Evaluate LLMs' ability to identify drug indications from natural language prompts & Expert-annotated correctness score \\


\href{https://github.com/knowlab/MedExQA}{MedExQA} & Medical & Evaluate LLMs' medical knowledge and explanation generation across underrepresented specialties & Explanation quality and expert-aligned LLM-judged relevance \\

\href{https://github.com/HanjieChen/ChallengeClinicalQA}{JAMA and Medbullets} & Medical & Evaluate LLMs' ability to answer and explain challenging clinical questions & Answer accuracy, explanation quality, and human-aligned reasoning assessment \\



\href{https://huggingface.co/datasets/TsinghuaC3I/MedXpertQA}{MedXpertQA} & Medical & Evaluate expert-level medical reasoning and multimodal clinical understanding across specialties & Answer accuracy, image-text reasoning performance, and expert-aligned scoring\\

\href{https://proceedings.neurips.cc/paper_files/paper/2024/file/9f80af32390984cb709cdeb014d0df41-Paper-Datasets_and_Benchmarks_Track.pdf}{MedJourney} & Medical & Evaluate LLM performance across full clinical patient journey stages and tasks & Task-specific automatic metrics (e.g., accuracy) and human expert evaluations \\


\href{https://github.com/gersteinlab/medagents-benchmark}{MedAgentsBench} & Medical & Evaluate complex multi-step clinical reasoning including diagnosis and treatment planning & Multi-aspect evaluation including correctness, efficiency, and human expert ratings \\


\href{https://github.com/kbressem/LongHealth}{LongHealth} & Medical (long-context) & Evaluate question answering over long-form clinical documents & Exact Match (EM), F1 score, and Long-Context QA accuracy \\

\href{https://github.com/JOHNNY-fans/MedOdyssey}{MedOdyssey} & Medical (long-context) & Evaluate long-context understanding in the Medical domain & Task-specific exact match, ROUGE, and human preference scoring \\


\midrule

\href{https://huggingface.co/datasets/openai/openai_humaneval}{HumanEval} & Code & Evaluate code generation, algorithmic reasoning, and language understanding with functional correctness & Test-case execution accuracy (pass@k) \\

\href{https://huggingface.co/datasets/Muennighoff/mbpp}{MBPP} & Code & Evaluate basic Python code generation on crowdsourced programming tasks & Functional correctness via pass@k using automated test cases \\


\href{https://huggingface.co/datasets/codeparrot/apps}{APPS} & Code & Evaluate coding challenge competence through real-world programming problems & Pass@k and exact match for functional correctness\\


\href{https://huggingface.co/datasets/xlangai/DS-1000}{DS-1000} & Code & Evaluate data science code generation across real-world queries from 7 Python libraries & Functional correctness via automated test-based execution accuracy \\


\href{https://github.com/microsoft/CodeXGLUE}{CodeXGLUE} & Code & Evaluate code understanding and generation across 9 tasks in 4 input-output types & Automatic metrics including BLEU, EM, F1, Accuracy, and MAP \\

\href{https://github.com/facebookresearch/cruxeval}{CruxEval} & Code & Evaluate code reasoning, understanding, and execution & pass@1 accuracy \\

\href{https://huggingface.co/datasets/neulab/odex}{ODEX} & Code & Evaluate cross-lingual code generation from natural language queries in four languages & Functional correctness via execution-based evaluation\\


\href{https://github.com/salesforce/CodeGen/tree/main/benchmark}{MTPB} & Code & Evaluate multi-turn program synthesis & Functional correctness via pass@k on step-wise subprograms \\

\href{https://huggingface.co/datasets/FudanSELab/ClassEval}{ClassEval} & Code & Evaluate class-level code generation from natural language descriptions in Python & pass@1, class completeness, dependency consistency, and error analysis \\

\href{https://huggingface.co/datasets/bigcode/bigcodebench}{BigCodeBench} & Code & Evaluate LLMs’ ability to follow complex instructions and invoke diverse function calls & Pass@k, test case execution accuracy, branch coverage \\


\href{https://huggingface.co/datasets/bigcode/humanevalpack}{HumanEvalPack} & Code & Evaluate multilingual code generation, correction, and comment synthesis across six programming languages & Functional correctness via pass@k and task-specific auto metrics \\


\href{https://github.com/bird-bench/mini_dev}{BIRD} & Code & Evaluate database-grounded text-to-SQL generation & Execution accuracy and exact match\\



\href{https://github.com/evalplus/repoqa}{RepoQA} & Code (long-context) & Evaluate long-context code understanding in real-world software repositories & Exact match accuracy and retrieval-augmented correctness\\

\href{https://github.com/JetBrains-Research/lca-baselines}{LongCodeArena} & Code (long-context) & Evaluate long-context code comprehension, generation, and editing across real-world tasks & Task-specific accuracy, exact match, and human evaluation\\



\midrule

\href{https://huggingface.co/datasets/openai/gsm8k}{GSM8K} & Math & Assess grade school math reasoning & Exact match accuracy \\

\href{https://huggingface.co/datasets/hendrycks/competition_math}{MATH} & Math & Evaluate mathematical problem-solving ability on competition-level questions with step-by-step reasoning & Final answer accuracy and step-wise derivation correctness \\


\href{https://huggingface.co/datasets/MathOdyssey/MathOdyssey}{MathOdyssey} & Math & Evaluate LLMs’ problem-solving capabilities on high school, university-level, and 
olympiad-level problems & Answer accuracy and performance across varying difficulty levels \\

\href{https://github.com/open-compass/MathBench}{MathBench} & Math & Evaluate theoretical understanding and practical application of mathematical knowledge across five levels & Accuracy on theoretical and application problems \\

\href{https://github.com/YilunZhou/champ-dataset}{CHAMP} & Math & Evaluate LLMs' fine-grained mathematical reasoning with concept and hint annotations on competition-level problems & Answer accuracy, reasoning path correctness\\


\href{https://huggingface.co/datasets/allenai/lila}{LILA} & Math & Evaluate LLMs’ mathematical reasoning across diverse formats and topics & Accuracy across 23 tasks \\


\href{https://github.com/openai/miniF2F}{MiniF2F-v1} & Math & Evaluate formal mathematical reasoning at Olympiad level & Proof accuracy on 488 problems\\

\href{https://huggingface.co/datasets/hoskinson-center/proofnet}{ProofNet} & Math & Evaluate auto-formalization and formal proof generation in undergraduate-level mathematics & Formalization accuracy and formal proof success rate in Lean 3 \\



\href{https://github.com/google-deepmind/alphageometry}{AlphaGeometry} & Math & Evaluate neuro-symbolic reasoning on olympiad-level Euclidean geometry theorems & Proof success rate, correctness, completeness, and human readability\\



\href{https://huggingface.co/datasets/AI4Math/MathVerse}{MathVerse} & Math & Evaluate MLLMs’ capability to interpret and reason over visual math diagrams & Diagram-sensitive answer accuracy with fine-grained CoT reasoning score\\

\href{https://huggingface.co/datasets/We-Math/We-Math}{We-Math} & Math & Evaluate LMMs’ visual mathematical reasoning with emphasis on knowledge acquisition and generalization & Four-dimensional diagnostic metrics\\

\href{https://huggingface.co/datasets/toloka/u-math}{U-MATH} & Math & Evaluate LLMs’ open-ended problem-solving skills across university-level math with visual components & Solution correctness judged by LLMs with expert-verified F1 score \\


\href{https://github.com/lupantech/PromptPG}{TabMWP} & Math & Evaluate mathematical reasoning over textual and tabular data & Accuracy on QA and multiple-choice questions \\


\href{https://github.com/SalesforceAIResearch/MathHay}{MathHay} & Math (long-context) & Evaluate long-context mathematical reasoning with multi-step dependencies & Accuracy, exact match, and reasoning chain consistency \\


\midrule

\href{https://huggingface.co/datasets/nguha/legalbench}{LegalBench} & Law & Evaluate legal reasoning across six types including rule application and interpretation & Task-specific accuracy, rule-consistency, and LLM-as-a-judge ratings \\

\href{https://huggingface.co/datasets/coastalcph/lex_glue}{LexGLUE} & Law & Evaluate legal language understanding across classification and QA tasks & Task-specific accuracy and F1 score (Auto) \\

\href{https://huggingface.co/datasets/joelniklaus/lextreme}{LEXTREME} & Law & Evaluate multilingual and multitask legal language understanding across 24 languages and 18 tasks & Task-specific accuracy, macro-F1, and classification metrics (Auto) \\


\href{https://github.com/open-compass/LawBench}{LawBench} & Law & Evaluate Chinese legal LLMs across retention, understanding, and application dimensions via 20 tasks & Task-specific accuracy and F1 \\

\href{https://github.com/Dai-shen/LAiW}{LAiW} & Law & Evaluate Chinese legal LLMs across fundamental, basic, and advanced legal tasks & Task-specific accuracy and F1 across 13 assignments \\

\href{https://huggingface.co/datasets/CSHaitao/LexEval}{LexEval} & Law & Evaluate LLMs' Chinese legal understanding and reasoning using a taxonomy of legal cognitive abilities & Task-specific accuracy\\

\href{https://arxiv.org/abs/2412.14556}{CitaLaw} & Law & Evaluate LLMs’ ability to generate legally sound answers with appropriate citations using statutes and precedent cases & Syllogism-based alignment score, citation accuracy and legal consistency \\

\href{https://github.com/CSHaitao/LegalAgentBench}{LegalAgentBench} & Law & Evaluate LLM agents’ ability to solve complex real-world legal tasks & Task success rate and intermediate progress rate \\


\href{https://github.com/vr18ub/court_view_generation}{SCALE} & Law (long-context) & Evaluate LLMs' legal reasoning across languages, long documents, and multitask legal scenarios & Accuracy, F1, and code-based assessment for long-context legal tasks \\


\midrule[0.5pt]
\bottomrule[1pt]
\end{tabular}
}
\end{table}

==> TMLR_Survey/Table/Table_selective_tuning.tex <==
\begin{table}[!t]
\small
\caption{\textbf{Selective-based Tuning.}}
% \vspace{2pt}
\centering
\renewcommand{\arraystretch}{1.3} 
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule[1pt]
\multirow{2}{*}{\textbf{Method}}& \multicolumn{4}{c}{\textbf{Challenge}}  \\  

\cmidrule{2-5}

& \textbf{Comm.} & \textbf{Non-IID} & \textbf{Memory} & \textbf{Comp.}   \\ 

\midrule[1pt]
% FedTT~\cite{ghiasvand2024communication}&\hlg{\tmark{}}&\hlg{\tmark{}}&&\\
{DP-BiTFiT~\cite{bu2022differentially}}\\
{FedPEFT~\cite{sun2022conquering}}\\
{RaFFM~\cite{yu2023bridging}}\\
{Selective FT~\cite{sun2024exploring}}\\


\bottomrule[1pt]
\end{tabular}
}
\label{Selective_tuning_table}
\end{table}

==> TMLR_Survey/Table/table_PEFT.tex <==

\begin{figure*}[!h]
    \centering
    \tikzset{
        basic/.style  = {draw, text width=3cm, rounded corners=1.5pt, align=center, font=\scriptsize, rectangle},
        root/.style   = {basic, thin, align=center, fill=mycolor_pink, text width=1.5cm},
        l1node/.style = {basic, thin, align=center, fill=mycolor_blond!20, text width=1.5cm},
        l2node/.style = {basic, thin, align=left, fill=mycolor_yellow, text width=4em, align=center},
        l3node/.style = {basic, thin, align=center, fill=mycolor, text width=3.cm},
        leaf/.style = {basic, thin, align=center, fill=mycolor_green, text width=12.6cm},
        leaf2/.style = {basic, thin, align=center, fill=mycolor_green, text width=8.8cm},
        wide leaf/.style = {basic, thin, align=left, fill=mycolor_green, text width=26.6em},
        edge from parent/.style={draw=black, edge from parent fork right}
    }
    \begin{forest}
        for tree={
            edge path={\noexpand\path[\forestoption{edge},->, line width=0.2mm] 
                (!u.parent anchor) -- +(4pt,0pt) |- (.child anchor)
                \forestoption{edge label};},
            grow=east,
            reversed=true,
            anchor=base west,
            parent anchor=east,  
            child anchor=west,  
            base=center,
            font=\small,
            rectangle,
            draw=black,
            rounded corners,
            align=center,
            minimum width=4em,
            edge+={semithick, draw=black,line width=0.5pt},
            s sep=2pt,
            l sep=12pt,
            inner xsep=4pt,
            inner ysep=4pt,
            scale=0.8, % 缩放树形图
            transform shape % 启用形状转换，保证缩放
        }
        % 树形图内容
        [Federated \\Fine-tuning, root
        [{LoRA-based \\ Tuning (\S\ref{sec_lora})}, l1node,  
        [Homogeneous \\ LoRA, l2node, 
                % [
                % Memory Efficiency, l3node,
                % [{
                % \textit{FedRA~\cite{su2023fedra}}},leaf2
                % ]
                % ]
                [
                    {\textit{FedIT~\citep{zhang2024towards}},  \textit{FedSA-LoRA~\citep{guo2024selective}}, \\
                    \textit{FederatedScope-LLM~\citep{fsllm}}, 
                    \textit{FeDeRA~\citep{yan2024federa}}, \textit{LoRA-FAIR~\citep{bian2024lora}},\\ \textit{FLASC~\citep{kuo2024federated}}, \textit{SA-FedLora~\citep{yang2024sa}}, 
                    \textit{SLoRA~\citep{babakniya2023slora}}, \textit{RoLoRA~\citep{chen2024robust}}, \\
                    \textit{FedPipe~\citep{fang2024automated}}, \textit{Lp-FL~\citep{lpfl}}, 
                    \textit{FedRA~\citep{su2023fedra}},\\
                    \textit{Fed-piLot~\citep{zhang2024fed}}, \textit{FedRA~\citep{su2023fedra}}
                    },leaf]
        ]
        [Heterogeneous \\ LoRA, l2node, 
                [
                    {\textit{HETLoRA~\citep{cho2024heterogeneous}}, \textit{FLoRA~\citep{wang2024flora}}
                    , \textit{FlexLoRA~\citep{bai2024federated}},
                    \textit{LoRA-A$^{2}$~\citep{koo2024towards}},\\
                    \textit{Replication-based Padding~\citep{byun2024towards}}, \textit{FedHM~\citep{yao2021fedhm}}, \textit{RBLA~\citep{tavallaie2024rbla}}
                    }, leaf]
        ]
        [Personalized\\ LoRA, l2node, 
                [
                {
                \textit{FDLoRA~\citep{qi2024fdlora}}, 
                \textit{pFedLoRA~\citep{yi2023fedlora}}, \textit{FedLoRA~\citep{wu2024fedlora}}, \textit{FedDPA~\citep{yang2024dual}},\\
                \textit{PerFIT~\citep{zhang2024personalized}}, \textit{FedMEM~\citep{du2024communication}},
                \textit{FedAMoLE~\citep{zhang2024personalized_new}}
                }, leaf]
        ]
    ]
    [{Prompt-based \\ Tuning (\S\ref{sec_prompt})}, l1node,  
        [General Prompt \\ Tuning, l2node, 
                [
                    {\textit{MetePFL~\citep{chen2023prompt}}, 
                    \textit{PromptFL~\citep{guo2023promptfl}},
                    \textit{FedBPT~\citep{sun2023fedbpt}},
                    \textit{FedPepTAO~\citep{che2023federated}},\\
                    \textit{Fed-BBPT~\citep{lin2023efficient}},
                    \textit{FedTPG~\citep{qiu2023text}}, 
                    \textit{FedPR~\citep{feng2023learning}},
                    \textit{Fed-CPrompt~\citep{bagwe2023fed}},\\
                    \textit{Fedprompt~\citep{zhao2023fedprompt}},
                    \textit{FedSP~\citep{dong2023tunable}},
                    \textit{HePCo~\citep{halbe2023hepco}},
                    \textit{PFL-GCN~\citep{ahmad2023prompt}},\\
                    \textit{AUG-FedPrompt~\citep{cai2023towards}},
                    \textit{\citet{liu2023federated}},
                    \textit{FedHPL~\citep{ma2024fedhpl}},
                    \textit{PFPT~\citep{wengprobabilistic}},\\
                    \textit{FCILPT~\citep{liu2023federated1}},
                    \textit{CaFPT~\citep{guo2024explore}},
                    \textit{FedPoD~\citep{chen2023federated2}}
                    },leaf]
        ]
    [Personalized\\ Prompt Tuning, l2node, 
                [
                    {\textit{pFedPG~\citep{yang2023efficient}}, 
                    \textit{SGPT~\citep{deng2024unlocking}}, 
                    \textit{pFedPrompt~\citep{guo2023pfedprompt}},
                    \textit{FedOTP~\citep{li2024global}},\\
                    \textit{pFedPT~\citep{li2023visual}},
                    \textit{FedMGP~\citep{yu2024personalized}},
                    \textit{FedLPPA~\citep{lin2024fedlppa}},
                    \textit{FedPGP~\citep{cui2024harmonizing}},\\
                    \textit{FedPFT~\citep{wu2024tackling}},
                    \textit{\citet{wang2024personalized}},
                    \textit{pFedMoAP~\citep{luo2024mixture}},
                    \textit{CP$^2$GFed~\citep{gao2024cp}}
                    },leaf]
        ]
        [Multi-domain \\ Prompt Tuning, l2node, 
                [
                    {\textit{DiPrompT~\citep{bai2024diprompt}}, 
                    \textit{PFCR~\citep{guo2024prompt}},
                    \textit{Fed-DPT~\citep{wei2023dual}},
                    \textit{FedAPT~\citep{su2024federated2}}, \\
                    \textit{\citet{zhao2024breaking}},
                    \textit{FedDG~\citep{gong2024federated}},
                    \textit{CP-Prompt~\citep{feng2024cp}}
                    },leaf]
        ]
    ]
    [{Adapter-based \\ Tuning (\S\ref{sec_adapter})}, l1node
            [General \\ Adapter Tuning, l2node, 
                [
                    {\textit{FedAdapter~\citep{cai2023efficient}},
                    \textit{\citet{kim2023efficient2}}, \textit{FedTT+~\citep{ghiasvand2024communication}},
                    },leaf]
            ]
            [Personalized \\ Adapter Tuning, l2node, 
                [
                    {\textit{C2A~\citep{kim2023client}}, 
                    \textit{FedCLIP~\citep{lu2023fedclip}}
                    },leaf]
            ]
            [Multi-domain \\ Adapter Tuning, l2node, 
                [
                    {\textit{Fed-MNMT~\citep{liu2023communication}}, 
                    \textit{AdaFedSelecKD~\citep{feng2024adapter}},
                    \textit{FedDAT~\citep{chen2024feddat}}
                    },leaf]
            ]
            ]
    [Selective-based \\ Tuning (\S\ref{sec_selective}), l1node
                [Bias \\ Tuning, l2node, 
                [
                    {\textit{DP-BiTFiT~\citep{bu2022differentially}}, 
                    \textit{FedPEFT~\citep{sun2022conquering}}
                    },leaf]
            ]
                [Partial \\ Tuning, l2node, 
                [
                    {\textit{RaFFM~\citep{yu2023bridging}}, 
                    \textit{\citet{sun2024exploring}}
                    },leaf]
            ]
            ]
    [Other Tuning \\ Methods (\S\ref{sec_hybrid}), l1node
                [Zero-Order \\ Optimization, l2node, 
                [{\textit{FedKSeed~\citep{qin2023federated}}, \textit{FwdLLM~\citep{xu2024fwdllm}},
                \textit{ZooPFL~\citep{lu2023zoopfl}},
                \textit{FedMeZo~\citep{ling2024convergence}},\\
                \textit{SPRY~\citep{panchal2024thinking}},
                \textit{CYBER-0~\citep{neto2024communication}}
                    },leaf]
            ]
            [Split \\ Learning, l2node, 
                [
                    {\textit{FedBERT~\citep{tian2022fedbert}}, 
                    \textit{FedSplitBERT~\citep{lit2022federated}},
                    \textit{FedSplitX~\citep{shin2023fedsplitx}}
                    },leaf]
            ]
            [Model \\ Compression, l2node, 
                [
                    {\textit{FedBiOT~\citep{wu2024fedbiot}}
                    },leaf]
            ]
            [Data \\ Selection, l2node, 
                [
                    {\textit{FedHDS~\citep{qin2024federated}}
                    },leaf]
            ]
            ]
            ]
            [Level 1, l1node
                [Level 2, l2node]
            ]
        ]
    \end{forest}
    \caption{Overview of Parameter-efficient Federated Fine-tuning Methods. The figure provides a classification of various parameter-efficient fine-tuning methods used in FL, categorizing them based on their strategies.}
    \label{main_table}
\end{figure*}



==> TMLR_Survey/Table/table_new_PEFT.tex <==

\begin{figure*}
    \centering
    
    \tikzset{
        basic/.style  = {draw, text width=3cm, rounded corners=1.5pt, align=center, font=\scriptsize, rectangle},
        root/.style   = {basic, thin, align=center, fill=mycolor_pink, text width=1.5cm},
        l1node/.style = {basic, thin, align=center, fill=mycolor_blond!20, text width=1.5cm},
        l2node/.style = {basic, thin, align=left, fill=mycolor_yellow, text width=4em, align=center},
        l3node/.style = {basic, thin, align=center, fill=mycolor_green, text width=3.cm},
        leaf/.style = {basic, thin, align=center, fill=mycolor_green, text width=12.6cm},
        wide leaf/.style = {basic, thin, align=left, fill=mycolor_green, text width=26.6em},
        edge from parent/.style={draw=black, edge from parent fork right}
    }

    \begin{forest}
        for tree={
            edge path={\noexpand\path[\forestoption{edge},->, line width=0.2mm] 
                (!u.parent anchor) -- +(4pt,0pt) |- (.child anchor)
                \forestoption{edge label};},
            grow=east,
            reversed=true,
            anchor=base west,
            parent anchor=east,  
            child anchor=west,  
            base=center,
            font=\small,
            rectangle,
            draw=black,
            rounded corners,
            align=center,
            minimum width=4em,
            edge+={semithick, draw=black,line width=0.5pt},
            s sep=2pt,
            l sep=12pt,
            inner xsep=4pt,
            inner ysep=4pt,
            scale=0.8, % 缩放树形图
            transform shape % 启用形状转换，保证缩放
        }
        % 树形图内容
        [Federated \\Fine-tuning, root
            [{LoRA-based \\ Tuning (\S\ref{sec_lora})}, l1node,  
        [General \\ LoRA Tuning, l2node, 
                [
                    {\textit{FedIT~\cite{zhang2024towards}}, \textit{FedTT~\cite{ghiasvand2024communication}}, \textit{FedSA-LoRA~\cite{guo2024selective}}, \textit{FeDeRA~\cite{yan2024federa}},\\ \textit{LoRA-FAIR~\cite{bian2024lora}}, \textit{FLASC~\cite{kuo2024federated}}, \textit{SA-FedLora~\cite{yang2024sa}}, \textit{SLoRA~\cite{babakniya2023slora}},\\ \textit{RoLoRA~\cite{chen2024robust}}, \textit{FedPipe~\cite{fang2024automated}}, \textit{Lp-FL~\cite{lpfl}}, \textit{LoRA-A$^{2}$~\cite{koo2024towards}},\\
                    \textit{FedRA~\cite{su2023fedra}},
                    \textit{Fed-piLot~\cite{zhang2024fed}}
                    },leaf]
        ]
        [Data\\Heterogeneous, l2node, 
                [
                    {\textit{HETLoRA~\cite{cho2024heterogeneous}}, \textit{FLoRA~\cite{wang2024flora}}
                    , \textit{FlexLoRA~\cite{bai2024federated}}, \textit{HAFL~\cite{su2024federated}},\\
                    \textit{Replication-based Padding~\cite{byun2024towards}}, \textit{FedHM~\cite{yao2021fedhm}}, \textit{RBLA~\cite{tavallaie2024rbla}}
                    }, leaf]
        ]
        [Memory\\ Wall, l2node, 
                [
                    {\textit{FDLoRA~\cite{qi2024fdlora}}, 
                \textit{pFedLoRA~\cite{yi2023fedlora}}, \textit{FedLoRA~\cite{wu2024fedlora}}, \textit{FedDPA~\cite{yang2024dual}},\\
            \textit{PerFIT~\cite{zhang2024personalized}}, \textit{FedMEM~\cite{du2024communication}}
                }, leaf]
        ]
    ]
    [{Prompt-based \\ Tuning (\S\ref{sec_prompt})}, l1node,  
        [ General Prompt \\ Tuning, l2node, 
                [
                    {\textit{MetePFL~\cite{chen2023prompt}}, 
                    \textit{PromptFL~\cite{guo2023promptfl}},
                    \textit{FedBPT~\cite{sun2023fedbpt}},
                    \textit{FedPepTAO~\cite{che2023federated}},\\
                    \textit{Fed-BBPT~\cite{lin2023efficient}},
                    \textit{FedTPG~\cite{qiu2023text}}, 
                    \textit{FedPR~\cite{feng2023learning}},
                    \textit{Fed-CPrompt~\cite{bagwe2023fed}},\\
                    \textit{Fedprompt~\cite{zhao2023fedprompt}},
                    \textit{FedSP~\cite{dong2023tunable}},
                    \textit{HePCo~\cite{halbe2023hepco}},
                    \textit{PFL-GCN~\cite{ahmad2023prompt}},\\
                    \textit{AUG-FedPrompt~\cite{cai2023towards}},
                    \textit{Fed-SP-SC~\cite{liu2023federated}},
                    \textit{FedHPL~\cite{ma2024fedhpl}},
                    \textit{PFPT~\cite{wengprobabilistic}},\\
                    \textit{FCILPT~\cite{liu2023federated1}},
                    \textit{CaFPT~\cite{guo2024explore}},
                    \textit{FedPoD~\cite{chen2023federated2}}
                    },leaf]
        ]
    [Personalized\\ Prompt Tuning, l2node, 
                [
                    {\textit{pFedPG~\cite{yang2023efficient}}, 
                    \textit{SGPT~\cite{deng2024unlocking}}, 
                    \textit{pFedPrompt~\cite{guo2023pfedprompt}},
                    \textit{FedOTP~\cite{li2024global}},\\
                    \textit{pFedPT~\cite{li2023visual}},
                    \textit{FedMGP~\cite{yu2024personalized}},
                    \textit{FedLPPA~\cite{lin2024fedlppa}},
                    \textit{FedPGP~\cite{cui2024harmonizing}},\\
                    \textit{FedPFT~\cite{wu2024tackling}},
                    \textit{Gradient-free~\cite{wang2024personalized}},
                    \textit{pFedMoAP~\cite{luo2024mixture}},
                    \textit{CP$^2$GFed~\cite{gao2024cp}}
                    },leaf]
        ]
        [Multi-domain \\ Prompt Tuning, l2node, 
                [
                    {\textit{DiPrompT~\cite{bai2024diprompt}}, 
                    \textit{PFCR~\cite{guo2024prompt}},
                    \textit{Fed-DPT~\cite{wei2023dual}},
                    \textit{FedAPT~\cite{su2024federated2}}, \\
                    \textit{Multilingual-FedPT~\cite{zhao2024breaking}},
                    \textit{FedDG~\cite{gong2024federated}},
                    \textit{CP-Prompt~\cite{feng2024cp}}
                    },leaf]
        ]
    ]
    [{Adapter-based \\ Tuning (\S\ref{sec_adapter})}, l1node
            [General \\ Adapter Tuning, l2node, 
                [
                    {\textit{FedAdapter~\cite{cai2023efficient}},
                    \textit{Adapter-tuning~\cite{kim2023efficient2}}
                    },leaf]
            ]
            [Personalized \\ Adapter Tuning, l2node, 
                [
                    {\textit{C2A~\cite{kim2023client}}, 
                    \textit{FedCLIP~\cite{lu2023fedclip}}
                    },leaf]
            ]
            [Multi-domain \\ Adapter Tuning, l2node, 
                [
                    {\textit{Fed-MNMT~\cite{liu2023communication}}, 
                    \textit{ADAFEDSELECTKD~\cite{feng2024adapter}},
                    \textit{FedDAT~\cite{chen2024feddat}}
                    },leaf]
            ]
            ]
    [Selective-based \\ Tuning (\S\ref{sec_selective}), l1node
                [Bias \\ Tuning, l2node, 
                [
                    {\textit{DP-BiTFiT~\cite{bu2022differentially}}, 
                    \textit{FedPEFT~\cite{sun2022conquering}}
                    },leaf]
            ]
                [Partial \\ Tuning, l2node, 
                [
                    {\textit{RaFFM~\cite{yu2023bridging}}, 
                    \textit{Selective FT~\cite{sun2024exploring}}
                    },leaf]
            ]
            ]
        [Other Tuning \\ Methods (\S\ref{sec_hybrid}), l1node
                [Model \\ Compression, l2node, 
                [
                    {\textit{FedIT~\cite{zhang2024towards}}, 
                    },leaf]
            ]
                [Zero-Order \\ Optimization, l2node, 
                [
                    {\textit{FedIT~\cite{zhang2024towards}}, 
                    },leaf]
            ]
            [Split \\ Learning, l2node, 
                [
                    {\textit{FedIT~\cite{zhang2024towards}}, 
                    },leaf]
            ]
            ]
            ]
            [Level 1, l1node
                [Level 2, l2node]
            ]
        ]
    \end{forest}
\end{figure*}
